Meta Representation Learning with Contextual Linear Bandits

Meta-learning seeks to build algorithms that rapidly learn how to solve new learning problems based on previous experience. In this paper we investigate meta-learning in the setting of stochastic linear bandit tasks. We assume that the tasks share a low dimensional representation, which has been partially acquired from previous learning tasks. We aim to leverage this information in order to learn a new downstream bandit task, which shares the same representation. Our principal contribution is to show that if the learned representation estimates well the unknown one, then the downstream task can be efficiently learned by a greedy policy that we propose in this work. We derive an upper bound on the regret of this policy, which is, up to logarithmic factors, of order $r\sqrt{N}(1\vee \sqrt{d/T})$, where $N$ is the horizon of the downstream task, $T$ is the number of training tasks, $d$ the ambient dimension and $r \ll d$ the dimension of the representation. We highlight that our strategy does not need to know $r$. We note that if $T> d$ our bound achieves the same rate of optimal minimax bandit algorithms using the true underlying representation. Our analysis is inspired and builds in part upon previous work on meta-learning in the i.i.d. full information setting \citep{tripuraneni2021provable,boursier2022trace}. As a separate contribution we show how to relax certain assumptions in those works, thereby improving their representation learning and risk analysis.

==> neurips/commands.tex <==
\newtheorem{lemma}{Lemma}
\newtheorem{assumption}{Assumption}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{fact}{Fact}
\newtheorem{sublemma}{Lemma}[section]

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\opnorm}[1]{\left\lVert#1\right\rVert_{\rm op}}
\newcommand{\specnorm}[1]{\left\lVert#1\right\rVert_{\rm F}}
\newcommand{\nucnorm}[1]{\left\lVert#1\right\rVert_{\ast}}
\newcommand{\quotes}[1]{``#1''}
\newcommand{\inn}[2]{\ensuremath \langle #1, #2\rangle}
\newcommand{\iidsim}{\mathrel{\stackrel{\makebox[0pt]{\mbox{\normalfont\tiny i.i.d.}}}{\sim}}}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\newcommand{\ntrain}{\overline{N}}



\DeclareMathOperator*{\argmax}{\ensuremath{argmax}}
\DeclareMathOperator*{\argsup}{\ensuremath{argsup}}

\DeclareMathOperator*{\argmin}{\ensuremath{argmin}}
\DeclareMathOperator*{\arginf}{\ensuremath{arginf}}

\usepackage[most]{tcolorbox}
\newtcolorbox[auto counter,number within=section]{protocol}[1][]{
  enhanced,
  breakable,
  fonttitle=\scshape,
  title={Protocol \thetcbcounter},
  #1
}
%%% INLINE COMMENTS
\newcommand{\massi}[1]{{\color{orange} #1}}
\newcommand{\leo}[1]{{\color{blue} #1}}
\newcommand{\karim}[1]{{\color{red} #1}}


\usepackage[textwidth=2.0cm, textsize=tiny]{todonotes} % for writting
\newcommand{\MP}[2][]{\todo[color=orange!20,#1]{{\bf MP:} #2}}
\newcommand{\LC}[2][]{\todo[color=blue!20,#1]{{\bf LC:} #2}}
\newcommand{\KL}[2][]{\todo[color=red!20,#1]{{\bf KL:} #2}}

==> neurips/learn_repr.tex <==
\section{Learning the Representation}\label{Sec:ReprLearning}
In this section we consider the problem of estimating the hidden representation $\B$ by $\Bhat_T$. Before proposing our solution, we will estimate $\B$ by improving the approach by \cite{boursier2022trace,tripuraneni2021provable} that was originally proposed for the i.i.d. case. Then, in the second half of the section we will introduce our approach. Not only it relaxes the assumptions of \cite{boursier2022trace,tripuraneni2021provable} but also requires less computations and is agnostic to the value of the rank $r$.

Similarly to what has been done in \cite{boursier2022trace}, let us consider $\W_T = \B \A_T \in \reals^{d\times T}$ where $\A_T = [\alphabf_1,\dots,\alphabf_T]^\top$.
As it was also investigated in \cite{cella2022multi}, we consider the trace-norm estimator
\begin{equation}\label{Eq:What}
    \What_T \in \argmin_{\W \in \reals^{d\times T}}\left\{ \frac{1}{T \Nold} \sum_{t=1}^T \sum_{n=1}^{\Nold} \left(y_{t,n} - \langle \x_{t,n}, \w_{t,n} \rangle \right)^2+ \lambda_{\Nold} \norm{\W}_* \right\}.
\end{equation}
Now, we compute the following decomposition of $\What_T$ to obtain $\Bhat_T$:
\begin{align}
\label{eq:Bhatdecompose}
  \What_T=\Bhat_T \widehat{\bf{A}}_T,\quad \Bhat_T\in\reals^{d\times \rhat}\;\;\text{with}\;\; \Bhat_T^\top \Bhat_T = \I_{\rhat},\;\;\text{and}\;\; \widehat{\bf{A}}_T\in\reals^{\rhat\times T}.
\end{align}
Here we set $\rhat = \rho(\What_T)$ equal to the rank of matrix $\What_T$.\\
%\LC{What do we say about ${\tilde r}$? Is it correct to say: we set $\rhat = \rho(\What_T)$}
%\KL{You are correct. I replaced $\tilde{r}$ by $\rhat$.}
An alternative choice to estimate the representation is to follow the same approach of \cite{boursier2022trace}, which requires the knowledge of the rank $r$ of $\W$. It then consists in computing the closest rank $r$ approximation of $\What_T$: 
\begin{equation}\label{Eq:Wbar}
    \Wbar_T \in \argmin_{\W \in \reals^{d\times T}: \rho(\W)\leq r} \norm{\W - \What_T}_{\rm F}.
\end{equation}
Next we compute the following decomposition: 
\begin{align}
\label{eq:Bdecompose}
  \Wbar_T=\Bbar_T \Abar_T,\quad \Bbar_T\in\reals^{d\times r}\;\;\text{with}\;\; \Bbar_T^\top \Bbar_T = \I_r,\;\;\text{and}\;\; \Abar_T\in\reals^{r\times T}.
\end{align}
We will then use $\Bbar_T$ as an estimate of the representation $\B$ when learning the task $T+1$.

Before going on with the analysis we need to recall the restricted strong convexity (RSC) condition, a standard definition from high-dimensional statistics. Notice, that this was used by~\cite{cellaSparseMTL} for the multi-tasks stochastic linear bandits. Denote by $\Sigmabar = \mathrm{diag}(\Sigmabf,\ldots,\Sigmabf)\in\reals^{dT\times dT}$.
 
\begin{definition}[RSC($\overline{r}$) Condition]\label{Def:RSC}
Let $\overline{\W}\in \reals^{d\times T}$ admits singular value decomposition $\overline{\W}={\bf U}{\bf D}{\bf V}^\top$ , and let ${\bf U}^{\overline{r}}$ and ${\bf V}^{\overline{r}}$ be the submatrices formed by the top $\overline{r}$ left and right singular vectors, respectively.
%associated with the top $r$ singular values.
We say that the restricted strong convexity RSC($\overline{r}$) condition is met for the theoretical multi-task matrix $\Sigmabar\in\reals^{dT\times dT}$, with positive constant $\kappa(\Sigmabar,\overline{r})$ if
\[
\min\left\{
    \frac{\norm{\rm{Vec}(\Deltabf)}_{\Sigmabar}^2}{2 \norm{\rm{Vec}(\Deltabf)}_2^2}: \Deltabf \in \Ccal(\overline{r})
\right\} \geq \kappa(\Sigmabar,\overline{r}).
\]
We used $\rm{Vec}(\Deltabf)$ for the $\reals^{dT}$ vector obtained by stacking together the columns of $\Deltabf$, and $\Ccal(r)$ is defined as
\begin{equation}\label{Eq:Cset}
    \left\{ \Deltabf \in \reals^{d\times T}:\; \nucnorm{\Pi(\Deltabf)} \leq 3 \nucnorm{\Deltabf - \Pi(\Deltabf)}\right\},
\end{equation}
where $\Pi(\Deltabf)$ is the projection operator onto set $\Bcal:=\{\Deltabf\in\reals^{d\times T}: \rm{Row}(\Deltabf)\perp {\bf U}^{\overline{r}}, \rm{Col}(\Deltabf)\perp {\bf V}^{\overline{r}}\}$.
\end{definition}
We are now ready to present one of the main technical results of this paper. It allows to relax the invertibility assumption of the covariance matrix $\Sigmabf$ in \cite{tripuraneni2021provable,boursier2022trace}. Indeed, as it is proved in Lemma \ref{lem:invertibility} 
in the appendix, we only need $\Sigmabf$ to satisfy the RSC condition. Since the proof is quite technical we leave it in the appendix and write only the statement here.
\begin{lemma}
%Assume that $\lambda_{\tilde{r}}(\Sigmabf)$ (the $\tilde{r}$-th largest eigenvalue of $\Sigmabf$) satisfies $\lambda_{\tilde{r}}(\Sigmabf)>c$ for some numerical constant $c>0$. Then there exists a numerical constant $C>0$ such taht the $\tilde{r}$-th largest eigenvalue of $\Bhat^\top\widehat{\Sigma}_{n}\Bhat$ satisfies $\lambda_{\tilde{r}}(\Bhat^\top\widehat{\Sigma}_{n}\Bhat)>C$ with probability at least $1-e^{-x}$.
Let Assumptions \ref{Ass:BoundedNorms} and \ref{Ass:ArmsDistribution} be satisfied. Let $\Sigmabf$ satisfies the RSC($\bar{r}$) condition for some integer $\bar{r}\geq 1$ with constant $\kappa(\Sigmabf)$. Let $\overline{\mathbf{M}} \in \reals^{d\times \bar{r}}$ admits orthonormal column vectors. Then, there exists a numerical constant $C>0$ such that, for any $\delta\in(0,1)$, we have with probability at least $1-\delta$, for any %$n\geq N_0(x)$ with
$n\geq C \bar{r}\log(2KN\delta^{-1})$
% $$
% N_0(x):= C_{C_{\mathbf{z}}, \nu \omega_{\Xcal},\kappa(\Sigmabf),\max_{k\in [K]}\opnorm{\Sigmabf_k}} \left( \bar{r}(x+\log(2KN))\bigvee (x+\log(2KN))^2\right),
% $$
% %for some enough constant $C>0$ that can depend only on $C_{\mathbf{z}}$,
% we have with probability at least $1-e^{-x}$
$$
\lambda_{\bar{r}}(\overline{\mathbf{M}}^\top\widehat{\Sigmabf}_{n}\overline{\mathbf{M}})>\frac{\kappa(\Sigmabf)}{4\nu \omega_{\Xcal}}>0.
$$
% $$
% \lambda_{\tilde{r}}(\Bhat^\top\widehat{\Sigmabf}_{n}\Bhat)>\frac{\kappa(\Sigmabf)}{4\nu \omega_{\Xcal}}>0.
% $$
\end{lemma}
The proof of this result uses the Freedman’s inequality for matrix-martingale \citep{Oliveira2010ConcentrationOT} combined with a truncation argument on the norm of the arms. 

% At any iteration $n\in[N]$ at task $T+1$, we could follow the approach of \citep{boursier2022trace}\KL{This is the approach by Jordan?} to get an estimate to the representation $\B$. We first estimate $\Wbar_T$ as the closest rank $r$ matrix to $\W_T$
% \begin{equation}\label{Eq:Wbar}
%     \Wbar_T \in \argmin_{\W \in \reals^{d\times T}: \rho(\W)\leq r} \norm{\W_T - \What_T}_F.
% \end{equation}
% We will use the following decompositions 
% \begin{align}
% \label{eq:Bdecompose}
%   \Wbar_T=\Bbar_T \Abar_T,\quad \Bbar_T\in\reals^{d\times r}\;\;\text{with}\;\; \Bbar_T^\top \Bbar_T = \I_r,\;\;\text{and}\;\; \Abar_T\in\reals^{r\times T}.
% \end{align}
% and similarly
% \begin{align}
% \label{eq:Bhatdecompose}
%   \What_T=\Bhat_T \widehat{\bf{A}}_T,\quad \Bhat_T\in\reals^{d\times \tilde{r}}\;\;\text{with}\;\; \Bhat_T^\top \Bhat_T = \I_{\tilde{r}},\;\;\text{and}\;\; \widehat{\bf{A}}_T\in\reals^{\tilde{r}\times T}.
% \end{align}

% $\Wbar_T$ as $\Wbar_T=\Bbar_T \Abar_T$ where $\Bbar_T\in\reals^{d\times r}$, $\Abar_T\in\reals^{r\times T}$ and $\Bbar_T^\top\Bbar_T=\I_r$.



% We need to extend the result stated in Corollary 1 of \citep{boursier2022trace} to the non i.i.d. setting. \KL{Do we need to say that beforehand? I would mention this result in a discussion after Theorem 2 where we explain how we improve over this paper and the one by Jordan.}


\subsection{Controlling the Estimation Error}
In this section we will discuss how to derive the estimation error bound \eqref{Eq:OracleBound} for $\Bbar_T$ (and $\Bhat_T$). The considered approach follows a bias-variance analysis of the estimation error $\Bbar_T\alphahat_{T+1,n} - \B\alphabf_{T+1}$. The bias part is treated through a novel perturbation argument which is valid even in the high-dimensional setting $d>n$ as it does not requires the invertibility of $\Sigmabf$ contrarily to the prior works \citep{tripuraneni2021provable,boursier2022trace} in the i.i.d. setting. We will remove the subscript $T+1$ when not necessary. 


% Finally, according to standard perturbation theory \citep{cai2018rate}\KL{Maybe change the reference. Probably based on prior result by wedin or Davis and Kahan?}, we will use 
% \[
%     \norm{\Bbar^\top\B_{\bot}} = \sqrt{1 - \sigma_{\min}^2\left(\Bbar^\top\B\right)} = \sin\Theta\left(\Bbar, \B\right).
% \]



\begin{theorem}[Bias Term]\label{Thm:NewBias1}
Considering a sequence of random covariates $\left(\x_s\right)_{s=1}^n\in\reals^d$ satisfying Assumptions \ref{Ass:BoundedNorms}, \ref{Ass:ArmsDistribution} and \ref{Ass:subGaussnoise} where for any given policy $\pi$, $\x_s$ is $\Fcal_{s-1}$-measurable. For any $\delta\in (0,1)$, let
\begin{align}
\label{eq:N0cond1}
    % N_0(x):= C_{C_{\mathbf{z}},\max_{1\leq k \leq K } \left\lbrace\opnorm{\Sigma_{k}}^{1/2}\right\rbrace}\left(  r\bigvee (x+\log(N))\right),
    %C_{C_{\mathbf{z}}, \nu \omega_{\Xcal},\kappa(\Sigmabf),\max_{k\in [K]}\opnorm{\Sigmabf_k}} \left( r(x+\log(2KN))\bigvee (x+\log(2KN))^2\right).
    N_0(x):= C \left(  r\bigvee \log(N\delta^{-1}) \right),
\end{align}
for some large enough numerical constant $C>0$ that do not depend on $n,N,r,d,\delta$. 
Let the RSC($r$) condition be satisfied by $\Sigmabf$, then the matrix $\Bbar_T$ defined in \eqref{eq:Bdecompose} satisfies, with probability at least $1-\delta$, for any $N_0(\delta)\leq n \leq N$,
\begin{align}
\norm{\Bbar_T\alphahat_n - \Bbf\alphabf} &\leq C \left( \norm{\alphabf}\frac{\opnorm{\What_T - \W}}{\sigma_{r}\left(\W\right)}  + \left( \frac{\log(4N r\delta^{-1})}{n}  \bigvee \sqrt{ \frac{\log(4N r\delta^{-1})}{n} } \right)\sqrt{r} \right),
\end{align}
for some numerical constant $C>0$ that does not depend on $n,N,r,d,\delta$.
%$C = C(C_{\mathbf{z}},\max_{1\leq k \leq K } \left\lbrace\opnorm{\Sigma_{k}}\right\rbrace, \sigma, c_{\etab})$

% \begin{align*}
% \norm{\Bhat\alphahat_n - \Bbf\alphabf} &\lesssim \left(1+\frac{4\nu \omega_{\Xcal}\, (1\vee \max_{k\in [K]}\lbrace  \opnorm{ \Sigmabf_k }\rbrace)}{\kappa(\Sigmabf)}\right) \norm{\alphabf}\frac{\opnorm{\What_T - \W}}{\sigma_{r}\left(\W\right)}  + \frac{4\nu \omega_{\Xcal}}{\kappa(\Sigmabf)}?????? \sqrt{\frac{r}{n}}.
% \end{align*}
\end{theorem}

We next observe that a similar result can be obtained for matrix $\Bhat_T$. 
\begin{theorem}[Bias Term]\label{Th:NewBias2}
Let the RSC($cr$) condition be satisfied by $\Sigmabf$ for some large enough absolute constant $c\geq 1$. Recall that $N_0(\delta)$ is defined in \eqref{eq:N0cond1}. Then the matrix $\Bhat_T$ defined in \eqref{eq:Bhatdecompose} satisfies, with probability at $1-\delta$, for any $N_0(\delta)\leq n \leq N$,
%Let $\Bhat$ be the  orthonormal projection matrices satisfying $\sin(\Bbar,\B)\leq \beta \leq 1$, 
\begin{align*}
\norm{\Bhat_T\alphahat_n - \Bbf\alphabf} &\leq C
\left( \norm{\alphabf}\frac{\opnorm{\What_T - \W}}{\sigma_{r}\left(\W\right)}  + \left( \frac{\log(4N r\delta^{-1})}{n}  \bigvee \sqrt{ \frac{\log(4N r\delta^{-1})}{n} } \right)\sqrt{r} \right),
\end{align*}
for some numerical constant $C>0$ that does not depend on $n,N,r,d,\delta$.
% \begin{align*}
% \norm{\Bhat\alphahat_n - \Bbf\alphabf} &\leq C \left( \norm{\alphabf}\frac{\opnorm{\What_T - \W}}{\sigma_{r}\left(\W\right)}  + \left( \frac{\log(4Nr) + x}{n}  \bigvee \sqrt{ \frac{\log(4Nr) + x}{n} } \right)\sqrt{r} \right),
% \end{align*}
% for some numerical constant $C = C(C_{\mathbf{z}},\max_{1\leq k \leq K } \left\lbrace\opnorm{\Sigma_{k}}\right\rbrace,\kappa(\Sigmabf),  \sigma, c_{\etab})$.
\end{theorem}
\paragraph{Result Discussion.} The first approach to choose an approximate representation in \eqref{eq:Bhatdecompose} not only avoids the invertibility assumption of $\Sigmabf$ but it also bypasses the closest rank $r$ approximation step in \eqref{Eq:Wbar},  thereby allowing for the design of a complete rank agnostic strategy. On the other hand the incurred constants may be quite large, so we also present the second strategy in \eqref{eq:Bdecompose}, which does require knowledge of the rank but involves smaller constants. We also point out that the perturbation analysis used to prove Theorem \ref{Thm:NewBias1} and \ref{Th:NewBias2} remains valid in the i.i.d. setting; see App.~\ref{AppSec:NewBias} for a discussion.

Then we can use the following bound on $\norm{\What_T - \W}_{F}$ given in 
%\MP{possibly we use a strange bibstyle, it would look better with normal parenthesis and in any case should be [Lemma 1 and Prop. 1, Cella et al. 2022]} 
 \cite{cella2022multi}[Lemma 1 and Prop.~ 1]. Define for any $\delta>0$
$$
\ntrain_0(\delta): = C  \left((d+T) \bigvee \log(dTKN\delta^{-1})\right) \log(dTKN\delta^{-1}),
$$
for some numerical constant $C>0$ that does not depend on $n,N,\ntrain,r,d,K,\delta$.

%$C = C\left(\nu, \omega_\Xcal,c_\eta,\sigma,C_{\x},\kappa(\Sigmabar),\max_{1\leq k \leq K }\left\lbrace \opnorm{\Sigma_{k}}^{1/2}\right\rbrace, L\right)$.

We have, provided that $\ntrain\geq \ntrain_0(\delta)$, with probability at least $1-\delta$, 
%\lesssim_{c_\eta,\sigma,C_{\x},\kappa(\Sigmabar),\max_{1\leq k \leq K }\left\lbrace \opnorm{\Sigma_{k}}^{1/2}\right\rbrace}
\begin{align}
\label{eq:intermediaire-WhatW}
\norm{ \What_{T} - \W}_{\rm F}  =  \mathcal{O}\left( \sqrt{\frac{r}{\ntrain}} \left(  \sqrt{(T+d)} \bigvee  \sqrt{\log(\delta^{-1})}\right)\right).
\end{align}
The previous display combined with Theorems \ref{Thm:NewBias1} and \ref{Th:NewBias2} gives (up to a rescaling of the constants), for any $\delta\in (0,1)$, with probability at least $1-\delta$
\begin{align}
\label{eq:2ndterm}
    \norm{\Bbar_T\alphahat_n - \Bbf\alphabf} &\leq C_1\left[  \sqrt{\frac{r}{\ntrain}} \left(  \sqrt{(T+d)} \bigvee  \sqrt{\log(\delta^{-1})}\right) \bigvee \sqrt{\frac{r\log(Nr\delta^{-1})}{n}}  \right],\\
   \norm{\Bhat_T\alphahat_n - \Bbf\alphabf} &\leq C_2\left[  \sqrt{\frac{r}{\ntrain}} \left(  \sqrt{(T+d)} \bigvee  \sqrt{\log(\delta^{-1})}\right) \bigvee \sqrt{\frac{r\log(Nr\delta^{-1})}{n}}  \right] ,
\end{align}
with numerical constants $C_1,C_2>0$ that does not depend on $n,N,\ntrain,r,d,K,\delta$.

%$C_1 = C\left(c_\eta,\sigma,C_{\x},\kappa(\Sigmabar),\max_{1\leq k \leq K }\left\lbrace \opnorm{\Sigma_{k}}^{1/2}\right\rbrace, L,\sigma_r(\W)\right)>0$ and $C_2 = C\left(c_\eta,\sigma,C_{\x},\kappa(\Sigmabar),\max_{1\leq k \leq K }\left\lbrace \opnorm{\Sigma_{k}}^{1/2}\right\rbrace, L ,\sigma_r(\W)\right)>0$.

\subsection{Meta-Learning Linear Contextual Bandits}

\noindent We are now ready to combine the results obtained in these last two subsections. This allows us to control the meta-regret (\ref{Eq:LTLRegret}) using either $\Bbar_T$ or $\Bhat_T$ as an approximation for $\B$ in Algorithm \ref{Alg:Greedy}.

\begin{corollary}
\label{cor:main}
Let Assumptions \ref{Ass:BoundedNorms}, \ref{Ass:ArmsDistribution}, \ref{Ass:subGaussnoise} be satisfied. For any $\delta_1,\delta_2\in (0,1)$, let us assume that $\ntrain \geq \ntrain_0(\delta_1)$ with  
$$
\ntrain_{0}(\delta_1):= C  \left((d+T) \bigvee \log(dTK\ntrain\delta_1^{-1})\right) \log(dTK\ntrain\delta_1^{-1}),
$$
and
$$
\label{eq:N0cond2}
	N \geq N_0(\delta_2):= C \left(  r\bigvee \log(KN\delta_2^{-1})\right),
$$
for some large enough numerical constant $C>0$ that does not depend on $n,N,\ntrain,r,d,K,\delta_1,\delta_2$.

%$C = C\left(\nu, \omega_\Xcal,c_\eta,\sigma,C_{\x},\kappa(\Sigmabar),\max_{1\leq k \leq K }\left\lbrace \opnorm{\Sigma_{k}}^{1/2}\right\rbrace, L,\sigma_r(\W)\right)$.
% $$
% \label{eq:N0cond}
% 	N \geq N_0(\delta_2):= C_{C_{\mathbf{z}},\max_{1\leq k \leq K } \left\lbrace\opnorm{\Sigma_{k}}^{1/2}\right\rbrace}\left(  r\bigvee \log(N\delta_2^{-1})\right),
%     %C_{C_{\mathbf{z}}, \nu \omega_{\Xcal},\kappa(\Sigmabf),\max_{k\in [K]}\opnorm{\Sigmabf_k}} \left( r(x+\log(2KN))\bigvee (x+\log(2KN))^2\right).
% $$
%for some large enough numerical constant $C_{C_{\mathbf{z}},\max_{1\leq k \leq K } \left\lbrace\opnorm{\Sigma_{k}}\right\rbrace}>0$.\\
%\textcolor{red}{Introduce $n_{0}(x):= \propto r$ for the new task}.
If $N\leq \ntrain$, then with probability at least $1-\delta_1-\delta_2$ , %the following holds
\begin{equation}
    R(T,N) \leq \bigO\left(r\sqrt{N} \left(1 \vee \sqrt{\frac{d}{T}} \vee \sqrt{\frac{\log\left(2\ntrain/\delta_1\right)}{T}} \bigvee \log(KN/\delta_2) \right)\right).
  %  \frac{N}{\sqrt{N^{tr}}}
\end{equation}
\end{corollary}
%\MP{There is explicit dependency on $K$in (19)?}
%\KL{Indeed, $N_0$ depends logarithmically on $K$. See Lemma 4. I corrected.}
\paragraph{Result Discussion.} If we consider the standard $d$-dimensional linear contextual bandit setting, the regret minimax lower-bound is of order $d\sqrt{N}$ \cite[Thm. 24.2, Sec. 24.2]{lattimore2020bandit}. On the other hand, a policy, which uses the true representation $\B$, essentially works in a $r$-dimensional bandit setting and thus it will incur at best the minimax-optimal regret lower bound of $r\sqrt{N}$. For $T$ large enough ($\geq d$), our regret matches this minimax-optimal lower bound, hence we can state that our policy is optimal. {Notice also that the bound depends at most logarithmically in the number of arms $K$.}
%\MP{Small issue: I think now we are minimax optimal apart logs? because we have $N$ near $K$ inside the log}
\begin{proof}
We can now combine the result of Theorem \ref{Th:RegretUBound} with the ones presented in the last section. 
%We can then use \eqref{{eq:intermediaire-WhatW}} which was proved in \cite{cella2022multi} (See Equation (51) in the proof of Theorem 1).
According to \cite{cella2022multi} (See Equation (51) in the proof of their Theorem 1), if $\lceil 
\ntrain_0(\delta_1)\rceil \leq \Nold$, then, with probability at least $1-\delta_1$, 
\begin{equation}
\label{eq:intermediaire-WhatW_MTL}
%\norm{ \What_{T,\Nold} - \W_T}_{\rm F} \lesssim_{c_\eta,\sigma,C_{\x},\kappa(\Sigmabar),\max_{1\leq k \leq K }\left\lbrace \opnorm{\Sigma_{k}}^{1/2}\right\rbrace}  \sqrt{\frac{r}{\Nold}} \left(  \sqrt{(T+d)} \bigvee  \sqrt{\log(2\Nold\delta_1^{-1})}\right).
\norm{ \What_{T,\Nold} - \W_T}_{\rm F} \leq \bigO \left( \sqrt{\frac{r}{\Nold}} \left(  \sqrt{(T+d)} \bigvee  \sqrt{\log(2\Nold\delta_1^{-1})}\right) \right).
\end{equation}
%\MP{I meant to say that it does not look very nice, actually, without meaning to offend, it looks quite ugly! Can we simplify it?}
%\LC{I've commented the old one. Is it better now?}
% In the following inequality we rely on an intermediate result of Theorem 1 in \cite{cella2022multi} which holds with probability at least $1-\delta_1$,
% \begin{equation}\label{Eq:TraceNormBound}
%      \frac{\norm{\What_{T,N} - \W_T}^2_F}{T\nu} \lesssim \frac{1}{T \nu} \left[\sqrt{\frac{r}{N}}\left(\sqrt{T+d} + \sqrt{\log\left(\frac{2 N}{\delta}\right)}\right) \right]^2.%\bigO\left(\right)
% \end{equation}

% Hence, combining the results of Theorem \ref{Thm:NewBias}  and Equation (\ref{eq:intermediaire-WhatW}) we have $\norm{\Bbar^\top\B_\bot}^2 \lesssim \beta^2$ with
% \[
%     \beta^2 = \frac{Tr}{\Nold\nu} + \frac{dr}{T \Nold \nu} + \frac{r}{T\Nold\nu} \log\left(2\Nold\delta_2^{-1}\right).
% \]
Consequently, the following holds with probability at least $1-\delta_1-\delta_2$
\begin{align*}
	\sum_{n=1}^N &\gamma(T, n) \leq \sum_{n=N_0}^N Cr \Bigg[ \frac{\norm{\alphabf}}{\sigma_{r}\left(\W\right)} \sqrt{\frac{1}{\Nold\nu}} \left(1 + \sqrt{\frac{d}{T }} + \sqrt{\frac{1}{T} \log
	%\left(
	\frac{2\Nold}{\delta_1}
	%\right)
	} \right) + \\ 
	&\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad ~+ \Bigg( \frac{\log(4N r) + \log
	%(
	\frac{N}{\delta_2}
	%)
	}{n}  \bigvee \sqrt{ \frac{\log(4N r) + \log
	%(
	\frac{\ntrain}{\delta_1}
	%)
	}{n} } \Bigg) \Bigg]\\
	&\leq C'r \left[ \sqrt{\frac{N^2}{\ntrain}} \left(1 + \sqrt{\frac{d}{T }} + \sqrt{\frac{1}{T} \log
	%\left(
	\frac{2\Nold}{\delta_1}
	%\right)
	} \right) + \left(\log(4N r) + \log
	%\left(
	\frac{N}{\delta_2}
	%\right)
	\right) 2 \sqrt{N} \right].
\end{align*}
We define $N_0$ according to Lemma \ref{lem:invertibility} 
as the smallest $n\in[N]$ such that the invertibility of $\Bhat^\top\widehat{\Sigmabf}_{n}\Bhat$ or $\overline{\Bbf}^\top\widehat{\Sigmabf}_{n}\overline{\Bbf}$ is guaranteed w.h.p. Consequently the estimator in \eqref{Eq:alphahat} is uniquely defined and we can apply Theorem \ref{Thm:NewBias1} or \ref{Th:NewBias2}. Specifically, according to Lemma \ref{lem:invertibility}  we have
\[
%    N_0 \geq r  \frac{\max_{k\in[K]}\norm{\Sigma_k}}{\lambda_{\min}(\Sigmabf_n)} \geq \max\left( 2 r \nu \omega_{\Xcal} \frac{\max_{k\in[K]}\norm{\Sigma_k}}{\lambda_{\min}(\Sigmabf)}, \frac{C \textcolor{red}{b^2 d} \nu\omega_{\Xcal} (x + \log(dT))}{\lambda_{\min}(\Sigmabf)} \right),
        N_0(\delta_2)= 
        C\left(r\bigvee\log(KN\delta_2^{-1})\right),
\]
where $C>0$ can depend only on $C_{\mathbf{z}}$ and $\max_{1\leq k \leq K } \left\lbrace\opnorm{\Sigma_{k}}^{1/2}\right\rbrace$.
The statement follows by combining this result with Theorem \ref{Th:RegretUBound}.
\end{proof}

%\section{Discussion and Implications}
\section{Conclusions}
In this paper we have investigated the problem of meta-learning with contextual linear bandit tasks. We considered the  setting in which a low dimensional representation is shared among the tasks and the goal is to use the representation inferred from multiple past tasks to facilitate learning novel tasks in the future, which share the same representation. Sharp guarantees for this problem have been recently studied in the i.i.d. statistical setting \citep{tripuraneni2021provable,boursier2022trace}, but the bandit setting has received considerably less attention. Inspired by those works, we analysed the performance gain of a bandit policy which exploits an approximate representation, estimated by a previous multitask learning procedure, when learning a new downstream task.
%belongs to the same representation space but is is distinct from the training tasks. 
Specifically we showed that a simple greedy policy which uses the estimated representation satisfies a regret bound on the test task that depends on the estimation error of the representation and matches under certain conditions the bound of an optimal strategy which has full knowledge of the true representation. Our result also apply as a special case to the i.i.d. setting, offering a number of key improvements.
%we were also able to make the estimator proposed in \citep{boursier2022trace} more efficient. 

% \begin{theorem}\label{Th:EstErrorUB}[Bounding the Estimation Error] 
% At any round $n\in[N]$, let $\{\x_s: s \in [n]\}$ be the arm sequence generated by the greedy policy of Algorithm \ref{Alg:Greedy}. According to the previous notation, assuming $\norm{\Bbar^\top\B_{\bot}}\leq \beta$ holds with probability at least $1-\delta_1$ and $n\geq r \frac{\lambda_{\max}(\Sigmabf_n)}{\lambda_{\min}(\Sigmabf_n)}$; then the following holds
% \begin{equation}
%     \norm{\Bbar\alphahat_{n} - \B\alphabf} \leq \bigO\left(\beta + \sqrt{\frac{r}{n}}\right)
% \end{equation}
% with probability at least $1-\delta_1-\delta_2$.
% \end{theorem}


% \begin{proof}
% We consider the new task estimator $\alphahat_{n}$ defined in \eqref{Eq:alphahat}. Set $\X_n = (\x_1\vert \ldots\vert\x_n)^\top \in \reals^{n\times d}$ and $\y_{n}= (y_1,\ldots,y_n)^\top \in \reals^n$. In agreement with the linear model specified in (\ref{Eq:LinearReward}), we have
% \MP{where is matrix ${\bf X}_n$ defined? Do we need to assume $\Bbar^\top \X_{n}^\top \X_{n}\Bbar$ invertible?}
% \KL{I think we need to replace this formula by the pseudo-inverse. The matrix $\X_n$ is not defined.}
% \begin{align*}
%     \alphahat_{n} &= \left(\Bbar^\top \X_{n}^\top \X_{n}\Bbar\right)^{-1}\Bbar\X_{n}^\top \y_{n} = \left(\Bbar^\top \X_{n}^\top \X_{n}\Bbar\right)^{-1}\Bbar\X_{n}^\top \left(\X_{n}\B\alphabf + \etab_{n}\right).
% \end{align*}
% We can then decompose the estimation error as:
% \[
%     \Bbar\alphahat_{n} - \B\alphabf = \Bbar\left(\Bbar^\top \X_{n}^\top \X_{n}\Bbar\right)^{-1}\Bbar\X_{n}^\top \left(\X_{n}\B\alphabf + \etab_{n}\right)- \B\alphabf ,
% \]
% from which we can upper bound $\norm{\Bbar_T\alphahat_{n} - \B\alphabf}$ respectively by the following bias and variance terms:
% \[
%     \sqrt{2}\norm{\Bbar \left(\Bbar^\top \X_{n}^\top \X_{n}\Bbar\right)^{-1}\Bbar\X_{n}^\top \X_{n}\B\alphabf - \B\alphabf} + \sqrt{2}\norm{ \Bbar \left(\Bbar^\top \X_{n}^\top \X_{n}\Bbar\right)^{-1}\Bbar\X_{n}^\top \etab_{n}}.
% \]
% The proof finishes by controlling the variance term with Lemma \ref{Le:Variance} and the bias term with Lemma \ref{Le:Bias}.
% \end{proof}

% \begin{lemma}[Variance Term]\label{Le:Variance} Let us consider the sequence of $n$ covariates $\x_s$ and additive noise variables $\eta_s$ satisfying Assumption \ref{Ass:ArmsDistribution}, \ref{Ass:BoundedNorms}, \ref{Ass:subGaussnoise}. Then, if $\frac{n}{\log n} \geq r \left(\frac{ \lambda_{\max}(\Sigmabf_n)}{\lambda_{\min}(\Sigmabf_n)}\right)^2$ we have
% \begin{equation}
%     \norm{ \Bbar \left(\Bbar^\top \X_{n}^\top \X_{n}\Bbar\right)^{-1}\Bbar\X_{n}^\top \etab_{n}} \leq \bigO\left(\sqrt{\frac{r \log n}{\lambda_{\min}(\Sigmabf_n)n}}\right)
% \end{equation}
% with probability at least $1 - \delta_2$.
% \end{lemma}\KL{The proof of this lemma depends on a paper by Banerjeet al. which looks dubious to me.}
% \begin{proof}
% Similarly to \citep{tripuraneni2021provable}[Lemma 18], we first consider the following upper bound $\norm{\Bbar(\Bbar^\top\X_n^\top\X_n\Bbar)^{-1}\Bbar^\top\X_n^\top\etab}^2 \leq\norm{\left(\Bbar^\top \X_{n}^\top \X_{n}\Bbar\right)^{-1}\Bbar^\top\X_n^\top\etab}^2$. Differently from the i.i.d. case, here we need a different quadratic form holding for dependent data. Indeed, according to Assumption \ref{Ass:subGaussnoise}, the noise $\eta_s$ is subGaussian adapted to $\Fcal_{s-1}$. We need to rely on the data-dependent generalization of Hanson-Wright inequality (see \citep{banerjee2019random}[Theorem 5]). Hence, conditionally on $\X_n$ we have
% \[
%     \Pro\left[ \etab^\top \A \etab - \E\left[\etab^\top \A \etab\right] \geq t \right] \leq 2 \exp \left( -c \min\left( \frac{t^2}{\left(\norm{\A}_F\norm{\A}\right)}, \frac{t}{\norm{\A}}\right) \right),
% \]
% where $\A=\frac{1}{n} \frac{\X_n\Bbar}{\sqrt{n}} \Bbar \left(\Bbar^\top \frac{\X_n ^\top \X_n}{n} \Bbar\right)^{-2} \frac{\Bbar^\top \X_n^\top}{\sqrt{n}}$. Hence, $\etab^\top\A\etab\leq \E\left[\etab^\top \A \etab\right] + \bigO\left(\norm{\A}_F \sqrt{\log(2/\delta_1)}\right)+ \bigO\left(\norm{\A}\log(2/\delta_1)\right)$ with probability $\geq 1-\delta_1$. The rest follows by the same reasoning adopted in the proof of Lemma 18 in \citep{tripuraneni2021provable}.
% \MP{We may summarize the reasoning in the appendix?}
% \end{proof}

% \begin{lemma}[Bias Term]\label{Le:Bias}
% Considering a sequence of random covariates $\left(\x_s\right)_{s=1}^n\in\reals^d$ satisfying Assumption \ref{Ass:BoundedNorms}, where for any given policy $\pi$, $\x_s$ is $\Fcal_{s-1}$-measurable. Let $\B,\Bbar\in\reals^{r\times d}$ be rank $r$ orthonormal projection matrices satisfying $\sin(\Bbar,\B)\leq \beta \leq 1$, then if $\frac{n}{\log n}\geq \frac{\lambda_{\max}(\Sigmabf_n)}{\lambda_{\min}(\Sigmabf_n)}r$ we have
% \[
%     \norm{\Bbar \left(\Bbar^\top \X_{n}^\top \X_{n}\Bbar\right)^{-1}\Bbar\X_{n}^\top \X_{n}\B\alphabf - \B\alphabf} \leq \bigO\left(\norm{\alphabf}\frac{\lambda_{\max}(\Sigmabf_n)}{\lambda_{\min}(\Sigmabf_n)}\beta\right)
% \]
% with probability at least $1-\delta_2$.
% \end{lemma}
% \begin{proof}
%     Similarly to what has been done in Lemma 19 of \citep{tripuraneni2021provable} \MP{I'd cite Lemma 19 only once inside the proof}, to control this term we rely on the identity $\I_{d} = \Bbar \Bbar^{\top} + \Bbar_{\bot}^{\top} \Bbar_{\bot}$. Specifically, we have:
%     \begin{align*}
%         & \Bbar(\Bbar^\top\X^\top\X\Bbar)^{-1}\Bbar\X^\top\X\B\alphabf - \B \alphabf = (\Bbar_{\bot}\Bbar_{\bot}^{\top} - \I)\B \alphabf + \Bbar( \Bbar^\top\X^\top\X\Bbar )^{-1} \Bbar\X^\top\X\Bbar_{\bot} \Bbar_{\bot}^\top \B \alphabf \\
%         &=\Bbar_{\bot}\Bbar_{\bot}^\top\B\alphabf + \Bbar(\Bbar^\top\X^\top\X\Bbar)^{-1}\Bbar\X^\top \X \B^\top_{\bot} \B \alphabf \implies\\
%         &\norm{\Bbar(\Bbar^\top\X^\top\X\Bbar)^{-1}\Bbar\X^\top \X \B^\top_{\bot} \B \alphabf - \B \alphabf}^2 \leq 2 \left(\norm{\alphabf}^2 \beta^2 + \norm{(\Bbar^\top\X^\top\X\Bbar)^{-1}\Bbar\X^\top \X \B^\top_{\bot} \B \alphabf}^2 \beta^2 \norm{\alphabf}^2 \right).
%     \end{align*}
%     Now, considering the covariates $\left(\x_s\right)_{s=1}^n\in\reals^d$, where each $\x_s$ is $\Fcal_{s-1}$ measurable, we can rely on Lemma \ref{Le:QuadraticForm} to control the quantities $\C_1 = \Bbar^\top\frac{\X^\top\X}{n}\Bbar - \Bbar^\top\Sigmabf_n\Bbar$ and $\C_2 = \Bbar^\top\frac{\X^\top\X}{n}\B - \Bbar^\top\Sigmabf_n\B$.
%     Now, following the same reasoning of \citep{tripuraneni2021provable}[Lemma 19] and considering an union bound over the $N$ rounds, we have
%     $\norm{\left(\Bbar^\top\X^\top\X\Bbar\right)^{-1}\C_1}\leq \frac{1}{4}$ and $\norm{\C_1}\leq \bigO\left(\frac{\lambda_{\max}(\Sigmabf_n)}{\lambda_{\min}(\Sigmabf_n)}\sqrt{\frac{r \log n}{n}}\right)$ with probability $\geq 1 - \delta$. Applying Lemma 25 of \citep{tripuraneni2021provable} we also get $\left(\Bbar^\top\frac{\X^\top\X}{n}\Bbar\right)^{-1} = \left(\C_1 + \Bbar^\top \Sigmabf_n \Bbar \right)^{-1} = \left(\Bbar^\top \Sigmabf_n \Bbar \right)^{-1} + \F$ where $\norm{\F}\leq\frac{4}{3}\norm{\left(\Bbar^\top\Sigmabf_n\Bbar\right)^{-1}}\norm{\C_1\left(\Bbar^\top\Sigmabf_n\Bbar\right)^{-1}}$ with probability $\geq 1 - \delta$. A similar reasoning holds also for matrix $\C_2$. Finally, considering the intersection of these two events,
%     \begin{align*}
%         &\norm{\left(\Bbar^\top\frac{\X^\top \X}{n}\Bbar\right)^{-1}\Bbar^\top\frac{\X^\top\X}{n}\B} = \norm{\left((\Bbar^\top \Sigmabf_n \Bbar)^{-1} + \F \right) \left(\Bbar^\top \Sigmabf_n \B + \C_2 \right)} \leq \bigO\left(\frac{\lambda_{\max}\left(\Sigmabf_n\right)}{\lambda_{\max}\left(\Sigmabf_n\right)}\right)
%     \end{align*}
%     under the condition $n\geq r \log n \frac{\lambda_{\max}(\Sigmabf_n)}{\lambda_{\min}(\Sigmabf_n)}$.
% \end{proof}


% \begin{lemma}\label{Le:QuadraticForm}
% Considering a sequence of random covariates $\left(\x_s\right)_{s=1}^n\in\reals^d$ satisfying Assumption \ref{Ass:BoundedNorms}, where for any given policy $\pi$, $\x_s$ is $\Fcal_{s-1}$-measurable. Then, if $\A\in\reals^{r\times d}$ and $\B\in\reals^{r\times d}$ are both rank $r$ orthonormal projection matrices we have, for any $n\in N$
% \[
%     \norm{\A^\top\Sigmahat_n\B - \A^\top\Sigmabf_n\B} \leq \bigO\left(C_{\x}^2\left(\sqrt{\frac{r}{n}} + \sqrt{\frac{\log(N/\delta)}{n}} \bigvee \frac{r}{n} + \frac{\log(N/\delta)}{n} \right) \right)\footnote{The big O notation hides a multiplicative constant factor proportional to the subGaussian norm $C_{\x}$.}
% \]
% with probability at least $1-\delta$.
% \end{lemma}
% \begin{proof}
% Here we need to control the term $\norm{\A^\top\frac{\X^\top\X}{n}\B - \A^\top\Sigmabf_n \B}$, where the expectation is with respect to the policy (due to the noisy rewards) and not for the randomness of the decision sets.
% \begin{align*}
%     &\norm{\A^\top\Sigmahat_n\B - \A^\top\Sigmabf_n\B} = \norm{\A^\top\frac{\X^\top\X}{n}\B -  \A^\top\Sigmabf_n\B} =\frac{1}{n} \norm{\A^\top\X^\top_n\X_n\B - \A^\top \sum_{s=1}^n\E\left[\x_s\x_s^\top | \Fcal_{s-1} \right] \B}.
% \end{align*}
% Now we control it by relying on Bernstein's deviation inequality for martingales \citep{bercurio}[Theorem 3.14]. 
% \begin{align*}
%     \norm{\A^\top\X^\top_n\X_n\B - \A^\top \sum_{s=1}^n\E\left[\x_s\x_s^\top \lvert \Fcal_{s-1} \right] \B} &= \sup_{\ubf \in\Sb^{r-1},\vbf\in\Sb^{r-1}} \ubf^\top \A^\top \left[ \X^\top_n\X_n - \sum_{s=1}^n\E\left[\x_s\x_s^\top \lvert \Fcal_{s-1} \right] \right] \B \vbf\\
%     &= \sup_{\ubf \in\Sb^{r-1},\vbf\in\Sb^{r-1}} \ubf^\top \A^\top \M_n \B \vbf
% \end{align*}
% where we set $\M_0=\mathbf{0}_{d\times d}$. We now approximate the operator norm by considering $\Scal$, the $\epsilon$-cover of $\Sb^{r-1}$ which has cardinality at most $\left(\frac{3}{\epsilon}\right)^r$ \citep{vershynin2019}[Corollary 4.2.13]. Similarly to the first step of the proof of Theorem 4.4.5 in \cite{vershynin2019}, for $\epsilon=\frac{1}{5}$ we have,
% \[
%     \sup_{\ubf \in\Sb^{r-1},\vbf\in\Sb^{r-1}} \ubf^\top \A^\top \M_n \B \vbf \leq \frac{1}{1-3\epsilon} \sup_{\ubf \in\Scal,\vbf\in\Scal} \ubf^\top \A^\top \M_n \B \vbf.
% \]
% Using an union bound argument over the elements of the nets we also have
% \[
%     \Pro \left[ \sup_{\ubf \in\Sb^{r-1},\vbf\in\Sb^{r-1}} \ubf^\top \A^\top \M_n \B \vbf  \right] \leq 225^r \Pro \left[\sup_{\ubf \in\Scal,\vbf\in\Scal} \ubf^\top \A^\top \M_n \B \vbf \right].
% \]
% By construction $\left(\M_n\right)_{n\geq 0}$ is a square-root integrable martingale adapted to $\Fcal_{n-1}$. Hence, the same is true for $\Mtilde_n = \A^\top \M_n \B$. We can then define its corresponding increasing process by $\langle\Mtilde\rangle_0$. and for all $n\geq 1$ we have
% \begin{align*}
%     \langle\Mtilde\rangle_n = \sum_{s=1}^n \E\left[\left(\Mtilde_s - \Mtilde_{s-1}\right)^2 |\Fcal_{s-1}\right].
% \end{align*}
% We define for each $n\geq 1$,
% \begin{align*}
%     V_n &= \E\left[ \left( \Mtilde_n - \Mtilde_{n-1} \right)^2 | \Fcal_{n-1} \right] \leq \E\left[\left( \ubf^\top \A^\top \x_n\x_n^\top \B \vbf - \ubf^\top \A^\top \E\left[\x_n\x_n^\top | \Fcal_{n-1}\right] \B \vbf \right)^2 | \Fcal_{n-1} \right]\\
%     &\leq \E\left[\left( \ubf^\top \A^\top \x_n\x_n^\top \B \vbf \right)^2 | \Fcal_{n-1} \right] - \left(\ubf^\top \A^\top \E\left[\x_n\x_n^\top | \Fcal_{n-1}\right] \B \vbf \right)^2 \\
%     &\leq \E\left[\left(\ubf^\top \A^\top \x_n \x_n^\top \B \vbf \right)^2 | \Fcal_{n-1}\right].
% \end{align*}
% According to Assumption \ref{Ass:ArmsDistribution} and the definition of $C_{\x}$ we have
% \[
%     V_n \leq \E\left[\left(z_1 z_2\right)^2\right],
% \]
% where $z_1$ and $z_2$ are $C_{\x}$-subGaussian random variables. Hence, their product is subExponential with parameter $C^2_{\x}$ (see \cite{vershynin2019}[Lemma 2.7.6]). That being said, its second moment is upper bounded by $C^4_{\x}$ which gives
% \[
%     V_n \leq C^4_{\x}.
% \]
% In order to apply Bernstein's inequality \citep{bercurio}[see Theorem 3.14], we need to control the $p$-th moment of $\Delta\Mtilde_n$, where $\Delta\Mtilde_n$ is defined as
% \[
%     \Delta\Mtilde_n = \Mtilde_n - \Mtilde_{n-1} = \ubf^\top \A^\top \left( \x_n \x_n^\top - \E\left[\x_{n}\x_{n}^\top|\Fcal_{n-1}\right] \right) \B \vbf.
% \]
% Specifically, we have that for any $p\geq 3$ since we are handling a subExponential random variable  with parameter $C^2_{\x}$, the following holds
% \[
%     \Delta\Mtilde^p \leq (C^2_{\x} p)^p \leq (C^2_{\x} e)^p p! \leq p! \left(  C^4_{\x} \right) e^p \left( C^2_{\x}\right)^{p-2} \leq \frac{p!}{2} V_n c_2^{p-2}
% \]
% where we used $c_2 = e^3 C^2_{\x}$ and the second inequality holds thanks for Stirling's approximation. Finally, a combination of Theorem 3.14 in \cite{bercurio} and an union bound over the $N$ rounds gives the statement.
% \end{proof}

\bibliographystyle{plainnat}
\bibliography{reference}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerNA{}
%   \item Did you include the license to the code and datasets? \answerNA{}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> neurips/symbols.tex <==
\newcommand{\indep}{\perp \!\!\! \perp}
\newcommand{\0}{\mathbf{0}}
\newcommand{\RI}{\mathbf{RI}}
\newcommand{\alphabf}{\bm{\alpha}}
\newcommand{\alphahat}{\widehat{\bm{\alpha}}}
\newcommand{\alphatilde}{\widetilde{\bm{\alpha}}}
\newcommand{\abf}{\mathbf{a}}
\newcommand{\A}{\mathbf{A}}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Abar}{\overline{\mathbf{A}}}
\newcommand{\Atilde}{\widetilde{\Abf}}
\newcommand{\Bbf}{\mathbf{B}}
\newcommand{\bbarbf}{\overline{\mathbf{b}}}
%\newcommand{\bbar}{\overline{b}}
\newcommand{\bbar}{b}
\newcommand{\bbf}{\mathbf{b}}
\newcommand{\B}{\mathbf{B}}
\newcommand{\Bbar}{\overline{\mathbf{B}}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Bb}{\mathbb{B}}
\newcommand{\Bhat}{\widehat{\mathbf{B}}}
\newcommand{\Btilde}{\widetilde{\mathbf{B}}}
\newcommand{\Bias}{\mathrm{bias}}
\newcommand{\btilde}{\widetilde{\mathbf{b}}}
\newcommand{\bprime}{\mathbf{b}'}
\newcommand{\bzero}{\mathbf{0}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\C}{\mathbf{C}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Chat}{\widehat{C}}
\newcommand{\dtilde}{\widetilde{d}}
\newcommand{\dbar}{\overline{d}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Deltabf}{\mathbf{\Delta}}
\newcommand{\e}{\mathbf{e}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\epsilontilde}{\widetilde{\epsilon}}
\newcommand{\etab}{\pmb{\eta}}
\newcommand{\etabar}{\overline{\eta}}
\newcommand{\F}{\mathbf{F}}
\newcommand{\Fbar}{\overline{\mathcal{F}}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\h}{\mathbf{h}}
\newcommand{\Hbf}{\mathbf{H}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Hbar}{\mathbf{\overline{h}}}
\newcommand{\hhat}{\mathbf{\widehat{h}}}
\newcommand{\Htilde}{\widetilde{H}}
\newcommand{\ibar}{\overline{i}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\Ind}{\mathbb{I}}
\newcommand{\jbf}{\mathbf{j}}
\newcommand{\Jbar}{\overline{J}}
\newcommand{\Kcal}{\mathcal{K}}\newcommand{\K}{\mathcal{K}}
\newcommand{\lambdatilde}{\widetilde{\lambda}}
\newcommand{\lambdamin}{\lambda_{\min}}
\newcommand{\lambdamax}{\lambda_{\max}}
\newcommand{\mar}{\mathrm{Mar}}
\newcommand{\muhat}{\widehat{\mu}}
\newcommand{\M}{\mathbf{M}}
\newcommand{\Mtilde}{\widetilde{\M}}
\newcommand{\nat}{\mathbb{N}}
\newcommand{\nbar}{\overline{n}}
\newcommand{\op}{\textbf{op}}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\Otilde}{\widetilde{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Pbf}{\mathbf{P}}
\newcommand{\Phat}{\widehat{\Pbf}}
\newcommand{\Pro}{\mathbb{P}}
\newcommand{\Psitilde}{\widetilde{\Psi}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\rhat}{\widehat{r}}
\newcommand{\rbar}{\overline{r}}
\newcommand{\rn}{\overline{r}_n}
\newcommand{\rtn}{\overline{r}_{t,n}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Rbar}{\overline{R}}
\newcommand{\Shat}{\widehat{S}}
\newcommand{\Sigmabf}{\mathbf{\Sigma}}
\newcommand{\Sigmahat}{\widehat{\Sigmabf}}
\newcommand{\Sigmabar}{\overline{\Sigmabf}}
\newcommand{\Sigmabarhat}{\widehat{\overline{\Sigmabf}}}
\newcommand{\sigmamin}{\sigma_{\min}}
\newcommand{\sigmamax}{\sigma_{\max}}
\newcommand{\Sb}{\mathbb{S}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\tr}{\mathrm{Tr}}
\newcommand{\tbar}{\overline{t}}
\newcommand{\Tbar}{\overline{T}}
\newcommand{\ubf}{\mathbf{u}}
\newcommand{\uhat}{\widehat{\ubf}}
\newcommand{\utilde}{\widetilde{\ubf}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\Ubar}{\overline{\mathbf{U}}}
\newcommand{\vbf}{\mathbf{v}}
\newcommand{\V}{\mathbf{V}}
\newcommand{\var}{\text{Var}}
\newcommand{\vhat}{\widehat{\vbf}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Vbar}{\overline{\mathbf{V}}}
\newcommand{\Vhat}{\widehat{\mathbf{V}}}
\newcommand{\VbarTilde}{\widetilde{\overline{\mathbf{V}}}}
\newcommand{\ve}{\varepsilon}
\newcommand{\Vtilde}{\widetilde{\mathbf{V}}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\wstar}{\w^*}
\newcommand{\wbar}{\mathbf{\overline{w}}}
\newcommand{\what}{\mathbf{\widehat{w}}}
\newcommand{\W}{\mathbf{W}}
\newcommand{\What}{\widehat{\W}}
\newcommand{\whatbar}{\widehat{\overline{\mathbf{w}}}}
\newcommand{\wtilde}{\mathbf{\widetilde{w}}}
\newcommand{\Wtilde}{\widetilde{\mathbf{W}}}
\newcommand{\Wbar}{\overline{\mathbf{W}}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\xhat}{\widehat{\mathbf{x}}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\xtop}{\mathbf{x}^\top}
\newcommand{\xtilde}{\widetilde{\x}}
\newcommand{\xh}{\mathbf{x}^\mathbf{h}}
\newcommand{\xhtop}{\mathbf{x}^{\mathbf{h}\top}}
\newcommand{\xbar}{\overline{\mathbf{x}}}
\newcommand{\Xbar}{\overline{\mathbf{X}}}
\newcommand{\Xhat}{\widehat{\mathbf{X}}}
\newcommand{\Xhatbar}{\widehat{\Xbar}}
\newcommand{\Xtilde}{\widetilde{\mathbf{X}}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\yhat}{\widehat{y}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\Yhat}{\widehat{\mathbf{y}}}
\newcommand{\Yhatbar}{\widehat{\overline{\mathbf{y}}}}
\newcommand{\Ybar}{\overline{\mathbf{Y}}}
\newcommand{\ybar}{\overline{y}}
\newcommand{\Z}{\mathbf{Z}}
\newcommand{\Nold}{\overline{N}}
